MM-TTA: Multi-Modal Test-Time Adaptation for 3D Semantic Segmentation

Test-time adaptation approaches have recently emerged as a practical solution for handling domain shift without access to the source domain data. In this paper, we propose and explore a new multi-modal extension of test-time adaptation for 3D semantic segmentation. We find that directly applying existing methods usually results in performance instability at test time because multi-modal input is not considered jointly. To design a framework that can take full advantage of multi-modality, where each modality provides regularized self-supervisory signals to other modalities, we propose two complementary modules within and across the modalities. First, Intra-modal Pseudolabel Generation (Intra-PG) is introduced to obtain reliable pseudo labels within each modality by aggregating information from two models that are both pre-trained on source data but updated with target data at different paces. Second, Inter-modal Pseudo-label Refinement (Inter-PR) adaptively selects more reliable pseudo labels from different modalities based on a proposed consistency scheme. Experiments demonstrate that our regularized pseudo labels produce stable self-learning signals in numerous multi-modal test-time adaptation scenarios for 3D semantic segmentation. Visit our project website at https://www.nec-labs.com/~mas/MM-TTA.

==> figure/fig_arch/fig_teaser.tex <==
\begin{figure}
\begin{center}
\includegraphics[width=0.9\linewidth]{figure/fig_arch/teaser_ours.pdf}
% \vspace{1.0mm}
\caption{\textbf{Teaser (Initial)}}
\label{fig:teaser}
\end{center}
\end{figure}

==> section/9-backup.tex <==

\section{Introduction}

% Backup 

% Why Category 6D pose is Necessary
6D object pose estimation is one of the crucial tasks in various robotics and computer vision applications, such as robot manipulation and augmented reality (AR). To recognize and interact with objects in the 3D space, these applications require the types, sizes, locations, and orientations of the objects. For example, for a robot to grasp a mug, it needs to know what kind of a mug it is (type), how big or small the mug is (size), where the mug is exactly lying (location), and in what direction the handle of the mug is pointing (orientation). 
% In augmented reality, these kinds of information also enable virtual interaction with the objects re-rendered from the real world. The size information can be referred to as a metric scale object shape. The location and orientation of an object can be interpreted as a 6D object pose, with 3 degrees of freedom for each.

% Current Limitation of Category 6D pose Estimation [Obtaining Labeled data is difficult]
Recently, Category-level object pose estimation has been proposed by Wang~\etal~\cite{wang2019normalized}. 
%
%
\JS{While instance-level pose estimation studies requires prior knowledges, such as 3D CAD models and object's sizes, category-level pose estimation task do not depend on such priors.}
% Compared to instance-level pose estimation \cite{xiang2017posecnn,tremblay2018deep,wang2019densefusion}, this task assumes a 3D CAD model and size information of each object is unknown. 
%
%
Most of the methods relied on the RGB-D sensors with the real-world labeled dataset for training. However, obtaining a sufficient amount of labels to train 6D pose is laborious and costly, as it mostly relies on involving a large number of human annotators.

% Recent Works [6Dof]
% A few works \cite{wang2020self6d, zakharov2020autolabeling, zhang2021keypoint} tackle this problem in the pose estimation. Most of the methods\cite{wang2019normalized, Tian2020prior, chen2020cass} used 3D CAD or reconstructed the 3D shape and then did a high computational rendering process to generate pseudo label \cite{wang2020self6d, zakharov2020autolabeling}. Recently, Zhang \etal \cite{zhang2021keypoint} proposes the Keypoint-based pseudo keypoints label using RGB image in the instance level pose estimation without rendering process. Still, it is an open problem how to generate pseudo labels without human intervention using RGB-D data.

%  or auto-labeling strategy~\cite{}
\JS{A few studies~\cite{} has covered UDA for 6DoF using RGB data. However, these methods require high-computational rendering process for training and does not extend the possibilities in UDA for multi-modality domain,~\ie~RGB-D fusion. Still, it is an open problem how to generate pseudo labels without human intervention using RGB-D data.}

% Recent Works [UDA]

% Ours
To tackle this problem, we propose the RGB-D-based category-level object pose estimation pseudo-label framework. To clarify with recent works, our method does not rely on a high-computation rendering process and tackle multi-class using a single network. Contributions of this paper is summarized as:
\begin{itemize}
    \item We newly propose a simple UDA framework for category-level object pose estimation via RGB-D fusion.
    % \item Propose the joint augmentation for 2D/3D to train Robust teacher network.
    \item We reduce domain gaps in multi-modality (RGB and depth) through adaptive pseudo labels. % [RGB-D Fusion Pseudo Label]
    % \item Reduce the Domain Gap between Source  Domain Gap [Momentum, Adversarial Learning] 
    \item Extensive experiments demonstrate our general estimation in unmet environments and achieve state-of-the-art performance in ** dataset.
\end{itemize}
